JWST Advanced Deep Extragalactic Survey (JADES) Data Release 5: stellar population catalogue for galaxies in GOODS-N and GOODS-S

We present the galaxy stellar population catalogue from the JWST Advanced Deep Extragalactic Survey (JADES) Data Release 5 (DR5), providing homogeneous Bayesian inference of physical galaxy properties in GOODS-N and GOODS-S. Using deep JWST/NIRCam and MIRI imaging combined with ancillary multi-wavelength data, we model the spectral energy distributions of ~500,000 sources with the Prospector framework. Our modelling incorporates flexible non-parametric star-formation histories (SFHs), nebular emission, dust attenuation, metallicities, and mid-infrared AGN and dust emission. We adopt an evolving star-forming main sequence (SFMS) prior for modelling the SFHs, which provides a physically-motivated long-term shape of SFHs while retaining non-parametric flexibility. The prior links stellar mass growth and SFR through the observed redshift-dependent SFMS, shaping the global behaviour of the inferred SFHs but allowing substantial deviations and scatters wherever supported by the data. We derive posterior distributions for stellar masses, SFRs, SFHs, dust attenuation, metallicities, and AGN contributions. The depth and wavelength coverage of JADES enable robust stellar mass measurements down to low-mass limits, as well as improved constraints on recent star-formation activity for ~350,000 galaxies at z = 1 - 9. The adoption of a physically motivated prior mitigates unphysical solutions and reduces degeneracies between redshift, age, dust, and metallicity, particularly for faint sources. We validate the catalogue through consistency checks and comparison to spectroscopic redshifts where available. The resulting value-added catalogue provides a uniform set of stellar population parameters suitable for statistical studies of galaxy growth, quenching, and the build-up of stellar mass across cosmic time. The full catalogue and posterior summaries are publicly released as part of JADES DR5.

==> config/macros.tex <==
% EMAIL STUFF
\usepackage{etoolbox}
\makeatletter
\newcommand\sendemail[4]{%                %\newcommand\tpj@compose@mailto[3]{%
\edef\@tempa{mailto:#1?subject=#2&body=#3 }%
\edef\@tempb{\expandafter\html@spaces\@tempa\@empty}%
\href{\@tempb}{#4}}

\catcode\%=11
\def\html@spaces#1 #2{#1%20\ifx#2\@empty\else\expandafter\html@spaces\fi#2}
\catcode\%=14
\makeatother
% END EMAIL STUFF

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%% AUTHORS - PLACE YOUR OWN COMMANDS HERE %%%%%
\usepackage{adjustbox}
\usepackage{textgreek}
\usepackage{xargs}
\usepackage{xspace}

% Please keep new commands to a minimum, and use \newcommand not \def to avoid
% overwriting existing commands. Example:
\newcommand{\orcid}[2]{\href{http://orcid.org/#2}{#1}}
\newcommand{\orcidsymb}[2]{\href{http://orcid.org/#2}{#1\adjustbox{trim={-.15\width} {0\height} {-.15\width} {0\height},clip}{\includegraphics[height=10pt]{figs/orcid.pdf}}}}

\newcommand{\citationneeded}{\textcolor{ForestGreen}{$^{\rm citation\;needed}$}}
\let\oldtextsigma\textsigma
\renewcommand{\textsigma}{\oldtextsigma\xspace}
\let\oldtextdegree\textdegree
\renewcommand{\textdegree}{\oldtextdegree\xspace}
%\let\oldkms\kms
%\renewcommand{\kms}{\ensuremath{\mathrm{km\,s^{-1}}}\xspace}



%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%% %%%%%%%
%%%%%%%%% UNITS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%% %%%%%%%
\newcommand{\kms}{\ensuremath{\mathrm{km\,s^{-1}}}\xspace}
\newcommand{\Msun}{\ensuremath{{\rm M}_\odot}\xspace}
\newcommand{\Zsun}{\ensuremath{{\rm Z}_\odot}\xspace}
\newcommand{\yr}{\ensuremath{{\rm yr}}\xspace}
\newcommand{\Myr}{\ensuremath{{\rm Myr}}\xspace}
\newcommand{\Gyr}{\ensuremath{{\rm Gyr}}\xspace}
\newcommand{\peryr}{\ensuremath{{\rm yr^{-1}}}\xspace}
\newcommand{\Lsun}{\hbox{\,${\rm L}_\odot$}}
\newcommand{\kpc}{\text{kpc}\xspace}
\newcommand{\ZH}{\text{[Z/H]}\xspace}
\newcommand{\MUV}{\ensuremath{M_\mathrm{UV}}\xspace}
\newcommandx{\percm}[1][1=3]{\ensuremath{\mathrm{cm}^{-#1}}\xspace}	% per cm-squared

\newcommandx{\lambdar}[2][1=R,2=]{\ensuremath{\lambda_{\rm {#1}}{#2}}\xspace}
\newcommand{\eps}{\ensuremath{\epsilon}\xspace}
\newcommand{\mstar}{\ensuremath{M_\star}\xspace}
\newcommand{\mdyn}{\ensuremath{M_\mathrm{dyn}}\xspace}
\newcommand{\re}{\ensuremath{R_\mathrm{e}}\xspace}
\newcommand{\vstar}{\ensuremath{v_\star}\xspace}
\newcommand{\vnai}{\ensuremath{v_{\NaI}}\xspace}
\newcommand{\sigmastar}{\ensuremath{\sigma_\star}\xspace}
\newcommand{\sigmaestar}{\ensuremath{\sigma_{\star,\mathrm{e}}}\xspace}
\newcommand{\vperc}[1]{\ensuremath{v_{#1}}\xspace}

\newcommand{\vesc}{\ensuremath{v_\mathrm{esc}}\xspace}
%\newcommand{\nelec}{\ensuremath{\langle n_\mathrm{e}\rangle}\xspace}
\newcommand{\nelec}{\ensuremath{n_\mathrm{e}}\xspace}
\newcommand{\Telec}{\ensuremath{T_\mathrm{e}}\xspace}
\newcommand{\Rout}{\ensuremath{R_\mathrm{out}}\xspace}
\newcommand{\vout}{\ensuremath{v_\mathrm{out}}\xspace}
\newcommandx{\Mout}[2][1=,2=]{\ensuremath{M_{\mathrm{out}{#2}}^{#1}}\xspace}
\newcommandx{\Mdotout}[2][1=,2=]{\ensuremath{\dot{M}_{\mathrm{out}{#2}}^{#1}}\xspace}
\newcommand\sbullet[1][.5]{\mathbin{\vcenter{\hbox{\scalebox{#1}{$\bullet$}}}}}
\newcommand{\mbh}{\ensuremath{M_{\sbullet[0.85]}}\xspace}

\newcommandx{\fluxdcgs}[1][1=-20]{\ensuremath{\times 10^{#1}~\mathrm{erg\,s^{-1}\,cm^{-2}\,\AA^{-1}}}\xspace}
\newcommandx{\fluxcgs}[3][1=-20,2=\times,3=]{\ensuremath{{#2}10^{#1}~\mathrm{erg\,s^{{#3}-{#3}1}\,cm^{{#3}-{#3}2}}}\xspace}
\newcommandx{\powercgs}[2][1=44,2=\times]{\ensuremath{{#2}10^{#1}~\mathrm{erg\,s^{-1}}}\xspace}
\newcommandx{\ergs}{\ensuremath{\mathrm{erg\,s^{-1}}}\xspace}
\newcommand{\AV}{\ensuremath{A_V}\xspace}



%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%% %%%%%%%
%%%%%%%%% LINE SYMBOLS %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%% %%%%%%%

%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%% %%%%%%%
%%%%%%%%% Other symbols (unities, etc.) %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%% %%%%%%%

\newcommand{\cigale}{{\sc cigale}\xspace}
\newcommand{\jwst}{\textit{JWST}\xspace}
\newcommand{\hst}{\textit{HST}\xspace}
\newcommand{\ppxf}{{\sc ppxf}\xspace}
\newcommand{\prospector}{{\sc prospector}\xspace}
\newcommand{\emcee}{{\sc emcee}\xspace}
\newcommand{\eazy}{{\sc eazy}\xspace}
\newcommand{\cloudy}{{\sc cloudy}\xspace}
\newcommand{\pyneb}{{\sc pyneb}\xspace}
\newcommandx{\mappings}[1][1=]{{\sc mappings{#1}}\xspace}
\newcommand{\galfit}{{\sc galfit}\xspace}
\newcommand{\qubespec}{{\sc qubespec}\xspace}
\newcommand{\pysersic}{{\sc pysersic}\xspace}
\newcommand{\mpt}{{\sc mpt}\xspace}

\newcommand{\blackthunder}{BlackTHUNDER\xspace}
\newcommand{\Mdynvalue}{$\Mdyn = 2.0\pm0.5 \times 10^{11}$~\MSun}

\defcitealias{gordon+2003}{G03}

